Self-Orchestrating Language Models: Leveraging Semantic Dependence for Efficient Inference

Large language models (LLMs) demonstrate impressive capabilities, but their deployment presents significant efficiency challenges. Autoregressive decoding imposes substantial inference latency and under-utilizes hardware accelerators in low batch size regimes. Discrete diffusion models can generate in parallel but struggle to match autoregressive quality without many diffusion denoising steps. Long-context reasoning creates memory bottlenecks that strain even state-of-the-art accelerators. My thesis is that language models can direct their own inference execution strategy by annotating semantic dependence -- which tokens depend on which others -- in their generation. I call such models self-orchestrating language models. For each system, I design a runtime that acts on these annotations to parallelize autoregressive decoding, evict intermediate context, or derive denoising orders, achieving Pareto-optimal quality-efficiency trade-offs. I demonstrate this approach through three self-orchestrating systems. First, PASTA uses semantic dependence to parallelize autoregressive decoding, training the model to annotate which output chunks can generate independently. Second, TIP uses semantic dependence to evict intermediate reasoning steps from the KV cache, reducing memory consumption while preserving accuracy. Third, Planned Diffusion uses semantic dependence to derive a denoising order for discrete diffusion, autoregressively generating a plan that specifies which chunks to denoise in parallel.

==> defaultfonts.tex <==
% From mitthesis package
% Documentation: https://ctan.org/pkg/mitthesis

\ProvidesFile{mitthesis-defaultfonts.tex}[2025/09/23 v1.06 Load Computer/Latin Modern text and math fonts]

%% Default fonts
\ifpdftex
	\ClassNoteNoLine{\ClassName}{Loading Computer Modern text and math fonts (default for pdftex)}
	\RequirePackage[T1]{fontenc} % With T1 encoding, pdftex will silently load the cm-super fontset
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
	\RequirePackage{bm}
\else
	\ClassNoteNoLine{\ClassName}{Loading Latin Modern text and math fonts (default for unicode engines)}
	%
%   \RequirePackage[]{babel} % load babel (with desired options) if using a language other than English
    \RequirePackage[warnings-off={mathtools-colon,mathtools-overbracket},mathbf=sym]{unicode-math}
    % suppress warnings about lack of integration between mathtools and unicode-math.
    % Unicode-math loads fontspec package, but default fonts are not selected by fontspec in this case.
\fi

